Kinetic Field Theory for Cosmic Structure Formation

We apply kinetic field theory to non-linear cosmic structure formation. Kinetic field theory decomposes the cosmic density field into particles and follows their trajectories through phase space. We assume that initial particle momenta are drawn from a Gaussian random field. We place particular emphasis on the late-time, asymptotic behaviour on small spatial scales of low-order statistical measures for the distribution of particles in configuration and velocity space. Our main result is that the power spectra for density and velocity fluctuations in ensembles of particles freely streaming along Zel'dovich trajectories asymptotically fall off with wave number $k$ like $k^{-3}$ for $k\to\infty$, irrespective of the cosmological model and the type of dark matter assumed, with the exponent set only by the number of spatial dimensions. This conclusion remains valid for density-fluctuation power spectra if particle interactions are taken into account in a mean-field approximation. We also show that the bispectrum of freely-streaming particles falls off asymptotically like $k^{-11/2}$ under the same general conditions.

==> Makefile <==
SHELL	= /bin/bash
VPATH	= ./fig

figjpg	= fig_1a fig_1b fig_2 fig_6a fig_6b
figpdf	= fig_3 fig_4 fig_5 fig_7 fig_8 fig_17 fig_18 fig_19 fig_20

figures	= $(figjpg:=.jpg) $(figpdf:=.pdf)

default: figs main.pdf
figs:
	make -C fig

%.pdf: %.tex
	pdflatex $< > /dev/null 2>&1
	count=1; while test $$count -eq 1 ; do \
	pdflatex $< > /dev/null 2>&1; \
	count=`grep "Rerun to get" $*.log | wc -l`; \
	done
clean:
	make -C src clean
	make -C fig clean
	$(RM) *.{aux,log,out} *~
distclean: clean
	make -C src distclean
	make -C fig distclean
	$(RM) main.pdf

